The CAISAR Platform: Extending the Reach of Machine Learning Specification and Verification

The formal specification and verification of machine learning programs saw remarkable progress in less than a decade, leading to a profusion of tools. However, diversity may lead to fragmentation, resulting in tools that are difficult to compare, except for very specific benchmarks. Furthermore, this progress is heavily geared towards the specification and verification of a certain class of property, that is, local robustness properties. But while provers are becoming more and more efficient at solving local robustness properties, even slightly more complex properties, involving multiple neural networks for example, cannot be expressed in the input languages of winners of the International Competition of Verification of Neural Networks VNN-Comp. In this tool paper, we present CAISAR, an open-source platform dedicated to machine learning specification and verification. We present its specification language, suitable for modelling complex properties on neural networks, support vector machines and boosted trees. We show on concrete use-cases how specifications written in this language are automatically translated to queries to state-of-the-art provers, notably by using automated graph editing techniques, making it possible to use their off-the-shelf versions. The artifact to reproduce the paper claims is available at the following DOI: https://doi.org/10.5281/zenodo.15209510

==> related.tex <==
The evolution of FM took the community from small validation tools and
fragmented specification languages, to more efficient tools, that were compared
and evaluated in dedicated competition events such as the SMT and Runtime
Verification Competitions (prompting the need for standardized specification
languages such as \smtl~\cite{barrett2016satisfiability}) and then served as
back-ends in more complex and modular verification platforms (such as
\yyy~\cite{filliatre2013why3}, \fc~\cite{baudin2021dogged} or
\key~\cite{ahrendt2016deductive}).
While still in its early stages, the renewed evolution of FM, this time to
target AI-based systems, is following a path that takes it to similar
milestones. In particular, the competition for the Verification of Neural
Network (\vnnc) {\cite{brix2023first}}, crystallized the need for a common
formal specification language.

A specification in \vnnl is usually equivalent to the following.
%
\maR{Is it equivalent or equisatisfaible? I have a doubt as this is the formula
  we usually want to prove valid, but we do so by means of (equi)satisfaibility.
  It may be useful to recall how we prove such a formula valid, in
  general.}{equivalent}
%
% Alban: I suggest dropping \mathcal{X} and \mathcal{Y}.
Given a vector $v \in \mathbb{R}^n$ of dimension $n$,
$v_c$ refers to the $c$th coordinate of $v$.
Let 
%$x \in \mathbb{R}^d$ %(resp. $y \in \mathbb{R}^p$)
%be an input %(resp. an output) 
%vector with notation $x_c$ mearning the $c-$th coordinate of $x$,
$f : \mathbb{R}^d \mapsto \mathbb{R}^p$ be a function representing an NN
that takes a $d$-dimensional vector as input
and returns a $p$-dimensional vector,
$\vec{K} \subseteq \{1,\dots,p\}$ be a (possibly empty) set of integers,
and $a,b \in \mathbb{R}^d$ and $c,d \in \mathbb{R}^p$ be vectors.
A \vnnl specification is then equivalent to the following formula:
\begin{equation*}
  \begin{aligned}
    \forall x \in
    \ \mathbb{R}^d.\
    \forall y \in \mathbb{R}^p.\ 
    y = f(x) \implies
    %a_i,b_i,c_j,d_j \in
    %(\mathbb{R}\times\mathbb{R}\times\mathbb{R}\times\mathbb{R}).\ f : x
    %\mapsto y 
    \\
    (\bigwedge_{i = 0 .. d} a_i \leq x_i \leq b_i) \implies
    (\bigwedge_{j =
      0 .. p} c_j \leq y_j \leq d_j 
      \land
      \bigwedge_{k \in \vec{K}} y_p \leq y_k),
  \end{aligned}
\end{equation*}
which specifies that if the input is within a box defined by $a$ and $b$,
the output should be within the box of $c$ and $b$ and the output $y_p$
should be lower than the output for all indices in $\vec{K}$.

THIS IS OUR TARGET SPECIFICATION

EXISTING SOLVERS

==> transformations.tex <==
\caisar is able to reason about SVMs by translating them into equivalent \nir.

An SVM is a classical machine learning algorithm used for classification.
Its output is a vector $y \in \mathbb{R}^m$
where $y_{cl}$ is the \emph{score} of class $cl \in \{1,\dots,m\}$.
First consider the binary case.
Each class $cl$ is associated with $k$ pairs
$\langle S_1,b_1\rangle,\dots,\langle S_k,b_k\rangle$
where $S_i \in \mathbb{R}^d$ is a \emph{support vector}
and $b_i$ is a \emph{bias}.
Given a (possibly non-linear) function $f: \mathbb{R} \rightarrow \mathbb{R}$,
the score $y_{cl}$ for input $x \in \mathbb{R}^d$ is computed
as $\sum_{i \in \{1,\dots,k\}} \ f(b_i + x \cdot S_i)$.
%
When the number $m$ of classes is greater than two,
the traditional approach is to use a \emph{one-versus-one} comparison (ovo).
The SVM performs a binary classification for each pair of classes
(with support vectors and biases tailored for this binary classification)
and then attributes a score of $1$ to the higher-scoring class and $0$ to the other one.
These scores are then added up for each class.

\caisar automatically translates each SVM into a \nir
that implements the operations described above.
For instance, the computation for one class of an SVM can be encoded as a
\nir similar to that of \figurename\ref{fig:ovoclass}. It can then be encoded into
another \nir in charge of aggregating the output classes (figure omitted due to
space constraint).
% with three classes would lead to the \nir of \figurename\ref{fig:ovo}
% where each `$cli$ v. $clj$' box would be replaced by another \nir encoding the
% linear operations (figure omitted due to space constraints).
% similar to that of \figurename\ref{fig:ovoclass}.
% Notice that the binary classification in Fig~\ref{fig:ovoclass} assumes
% that the first class has three support vectors while the second only has one.
Not all solvers support the same set of operators,
which may require different translations;
for instance in \figurename\ref{fig:ovoclass}, operator \kw{Gather}
which would have been convenient to extract parts of a tensor
has been replaced with \kw{MatMul} and a constant tensor omitted on the figure.

\declareshaperectxy{1}{1}{4}{1}
\declareshaperectxy{1}{1}{1}{3}
% \begin{figure}[ht]
%   \begin{center}
%   	\begin{tikzpicture}[ONNX/.style={fill=black!10,rounded corners},
%       -|-/.style={
%         to path={
%           (\tikztostart) -| ($(\tikztostart)!#1!(\tikztotarget)$) |- (\tikztotarget)
%           \tikztonodes
%         }
%       },
%       -|-/.default=0.5,
%       |-|/.style={
%         to path={
%           (\tikztostart) |- ($(\tikztostart)!#1!(\tikztotarget)$) -| (\tikztotarget)
%           \tikztonodes
%         }
%       },
%       |-|/.default=0.5,
%     ]
%       \node (I) [ONNX] at (0, 2) {\kw{Input}};
%       \node (K1) [ONNX, rectangle 1x1x1x3] at (2, 2.8) {$cl1$ v. $cl2$};
%       \node (K2) [ONNX, rectangle 1x1x1x3] at (2, 2.) {$cl1$ v. $cl3$};
%       \node (K3) [ONNX, rectangle 1x1x1x3] at (2, 1.2) {$cl2$ v. $cl3$};
%       \node (S1) [ONNX, rectangle 1x1x3x1] at (5, 3) {\kw{Add (1)}};
%       \node (S2) [ONNX, rectangle 1x1x3x1] at (5, 2) {\kw{Add (2)}};
%       \node (S3) [ONNX, rectangle 1x1x3x1] at (5, 1) {\kw{Add (3)}};
%       \node (G) [ONNX, rectangle 1x1x4x1] at (7,2) {\kw{Concat}};
%       \node (O) at (8.5,2) {};
%       % input to binary classifier
%       \foreach \K in {1,2,3} {
%         \draw[->] (I.east) to[-|-] (K\K.west);
%       }
%       % binary classifier to add
%       %\foreach\K/\A/\L/\D in {1/1/1/0.25,1/2/2/0.25,2/1/2/-0.25,2/3/1/-0.25,3/2/1/0.25,3/3/2/0.25} {
%       %  \draw[->] (K\K.east) -- ++(\D,0) to[-|-] (S\A.l\L);
%       %}
%       \draw[->] (K1.r2) to [-|-] (S1.l2);
%       \draw[->] (K1.r1) -- ++ (0.5,0) to [-|-] (S2.l2);       
%       \draw[->] (K2.r2) -- ++ (0.25,0) to [-|-] (S1.l1);
%       \draw[->] (K2.r1) -- ++ (0.25,0) to [-|-] (S3.l2);
%       \draw[->] (K3.r2) -- ++ (0.5,0) to [-|-] (S2.l1);
%       \draw[->] (K3.r1) to [-|-] (S3.l1);
%       % add to concat
%       \foreach \A/\B in {1/3,2/2,3/1} {
%         \draw[->] (S\A.east) to[-|-] (G.l\B);
%       }
%       \draw[->] (G.east) -- (O.west);
% 	  \end{tikzpicture}
%   \end{center}
%   \caption{Overall translation of ovo SMVs.}
% 	\label{fig:ovo}
% \end{figure}


\begin{figure}[t!]
  \begin{center}
    \begin{tikzpicture}[ONNX/.style={fill=black!10,rounded corners},
      -|-/.style={
      to path={
          (\tikztostart) -| ($(\tikztostart)!#1!(\tikztotarget)$) |- (\tikztotarget)
          \tikztonodes
        }
      },
      -|-/.default=0.5,
      |-|/.style={
      to path={
          (\tikztostart) |- ($(\tikztostart)!#1!(\tikztotarget)$) -| (\tikztotarget)
          \tikztonodes
        }
      },
      |-|/.default=0.5,
      ]
      \node (I) [ONNX] at (0, 2.5) {\kw{Input}};
      \node (K1) [ONNX] at (2, 3.) {\kw{MatMul}};
      \node (K2) [ONNX] at (2, 2.5) {\kw{MatMul}};
      \node (K3) [ONNX] at (2, 2.) {\kw{MatMul}};
      \node (K4) [ONNX] at (2, 1.5) {\kw{MatMul}};
      \node (F1) [ONNX] at (3.5, 3.) {$f$};
      \node (F2) [ONNX] at (3.5, 2.5) {$f$};
      \node (F3) [ONNX] at (3.5, 2.) {$f$};
      \node (F4) [ONNX] at (3.5, 1.5) {$f$};
      \node (P1) [ONNX, rectangle 1x1x3x1] at (4.5, 3.5) {\kw{Add}};
      \node (P2) [ONNX, rectangle 1x1x3x1] at (5, 2.75) {\kw{Add}};
      \node (Diff) [ONNX, rectangle 1x1x3x1] at (6.25, 2.5) {\kw{Sub}};
      \node (Sign) [ONNX, rectangle 1x1x1x3] at (7.5, 2.5) {\kw{Sign}};
      \node (MSign) [ONNX] at (8.75, 1.5) {\kw{Sub}};
      \node (+1) at (10,3.5) {to $cl$};
      \node (-1) at (10,1.5) {to $cl'$};

      % MatMul + f
      \foreach \A in {1,2,3,4} {
          \draw [->] (I.east) to[-|-] (K\A.west);
          \draw[->] (K\A.east) -- (F\A.west);
        }
      % 1st add
      %\foreach \A/\B in {1/2,2/1} {
      %    \draw[->] (F\A.east) to[-|-] (P1.l\B);
      %  }
      \draw[->] (F1.east) to[-|-] (P1.l2);
      \draw[->] (F2.east) to ++(0.1,0) to[-|-] (P1.l1);
      % 2nd add (is there a better way for the first branch?)
      \path let \p1 = ($(F3.east)!0.5!(P2.l1)$) in let \p2 = (P2.l2) in coordinate (F) at (\x1,\y2);
      \draw[->] (P1.east) -- ++(0.25,0) to[|-|] (F) -- (P2.l2);
      \draw[->] (F3.east) to[-|-] (P2.l1);
      % sub
      \draw[->] (P2.east) to[-|-] (Diff.l2);
      \draw[->] (F4.east) to[-|-] (Diff.l1);
      % sign
      \draw[->] (Diff.east) -- (Sign.west);

      % output.  Is there a simpler way for the first one?
      \path let \p1 = ($(Sign.r2)!0.5!(MSign.west)$) in let \p2 = (Sign.r2) in coordinate (F) at (\x1,\y2);
      \draw[->] (Sign.r2) -- (F) -- (F |- +1.west) -- (+1.west);
      \draw[->] (Sign.r1) to[-|-] (MSign.west);
      \draw[->] (MSign.east) -- (-1.west);
    \end{tikzpicture}
  \end{center}
  \caption{\nir representation of an SVM binary classification of $cl$ and $cl'$ followed by a binarization of the outcome.}
  \label{fig:ovoclass}
\end{figure}


==> transformations2.tex <==
\caisar is able to reason about Support Vector Machines (SVM) by translating
them into equivalent \nir.

An SVM is a classical machine learning algorithm used for classification.
Its output is a vector $y \in \mathbb{R}^m$
where $y_{cl}$ is the \emph{score} of class $cl \in \{1,\dots,m\}$.
First consider the binary case.
Each class $cl$ is associated with $k(cl)$ \emph{support vectors}
$S_{cl,1},\dots,S_{cl,k(cl)}$ (vectors of dimension $d$).
Furthermore, each support vector $S_{cl,j}$
is associated with a \emph{dual coefficient} $c^{cl'}_{cl,j}$ (a scalar)
and the pair of classes $(cl_1,cl_2)$ is associated with an \emph{intercept}
$i_{cl_1,cl_2}$ (also a scalar).
Given a (possibly non-linear) function $f$ from reals to reals,
the SVM classifies input $x$ as $cl_1$
iff

\begin{displaymath}
  \sum_{j \in \{1,\dots,k(cl_1)\}}\ (c^{cl_2}_{cl_1,j} * f(x \otimes S_{cl_1,j}))
  - \sum_{j \in \{1,\dots,k(cl_2)\}}\ (c^{cl_1}_{cl_2,j} * f(x \otimes S_{cl_2,j}))
  + i
\end{displaymath}

is positive
and $cl_2$ if it is negative
(the probability that it equals zero is negligible).

SVMs with more than two classes often use the one-versus-one (or \textsc{ovo}) scheme.
The SVM performs a binary classification for each pair $(cl,cl')$ of classes
with dual coefficients and intercept specific to this pair.
For each class $cl$, the SVM then outputs the number of times this class was selected
against the class it was paired against.
So, for $10$ classes, the output of an SVM would be a vector of $10$ integers
each between $0$ and $9$.
%that adds up to $45$ ($C^2_{10}$ or \emph{choose 2 in ten})%
It should be clear that this will sometimes lead to two (or more) classes sharing top score,
something that is typically unfrequent in the case of binary classification.

\begin{figure}[t!]
  \begin{center}
    \begin{tikzpicture}[ONNX/.style={fill=black!10,rounded corners},
      -|-/.style={
      to path={
          (\tikztostart) -| ($(\tikztostart)!#1!(\tikztotarget)$) |- (\tikztotarget)
          \tikztonodes
        }
      },
      -|-/.default=0.5,
      |-|/.style={
      to path={
          (\tikztostart) |- ($(\tikztostart)!#1!(\tikztotarget)$) -| (\tikztotarget)
          \tikztonodes
        }
      },
      |-|/.default=0.5,
      UNDERBRACE/.style={
          thick,
          decoration={
              brace,
              mirror,
              raise=0.5cm
            },
          decorate
        },
      ]
      \usetikzlibrary{snakes}
      \node (I) at (0, 0) {\kw{X}};
      \node (SV) at (1.5, 1) {$S$};
      \node (K) [ONNX] at (1.5, 0) {\kw{Gemm}};
      \node (Params) at (3, 1) {\begin{tabular}{c}Kernel\\params\end{tabular}};
      \node (F) [ONNX] at (3, 0) {$f$};
      \node (Duals) at (4.5, 1) {$c$};
      \node (Sum) [ONNX] at (4.5, 0) {\kw{Gemm}};
      \node (Int) at (6, 1) {$i$};
      \node (Intercept) [ONNX] at (6, 0) {\kw{Add}};
      \node (Sign) [ONNX] at (7.5, 0) {\kw{Sign}};
      \node (Scores) [ONNX] at (9, 0) {\kw{Gemm}};
      \node (Y) at (10.5, 0) {\kw{Y}};

      \draw[->] (I) to (K);
      \draw[->] (SV) to (K);
      \draw[->] (K) to (F);
      \draw[->] (Params) to (F);
      \draw[->] (F) to (Sum);
      \draw[->] (Duals) to (Sum);
      \draw[->] (Sum) to (Intercept);
      \draw[->] (Int) to (Intercept);
      \draw[->] (Intercept) to (Sign);
      \draw[->] (Sign) to (Scores);
      \draw[->] (Scores) to (Y);

      \draw [UNDERBRACE] (K.west) -- (F.east)
      node [pos=0.5,anchor=north,yshift=-0.55cm] {kernel computation};
      \draw [UNDERBRACE] (Sum.west) -- (Sign.east)
      node [pos=0.5,anchor=north,yshift=-0.55cm] {\phantom{pk}one vs. one\phantom{pk}};
      \draw [UNDERBRACE] (Scores.west) -- (Scores.east)
      node [pos=0.5,anchor=north,yshift=-0.55cm] {\phantom{pk}adding up scores\phantom{pk}};

    \end{tikzpicture}
  \end{center}
  \caption{\nir representation of an SVM.}
  \label{fig:ovo}
\end{figure}

The translation of an SVM to a \nir is illustrated in Fig.~\ref{fig:ovo}.
The first part computes the kernel
(products of the support vectors with the input, followed by the $f$ function).
The second part computes the one-vs-one comparison
(product of the kernel values with the dual ones,
followed by the addition of the intercept and the positivity check).
Finally, the last layer adds up the scores of each class.

\caisar currently supports Linear and Polynomial kernel functions. Radial Basis
Function (RBF) kernels support is planned for a future \caisar release.

% eof

